AsterixDB: A Scalable, Open Source BDMS

AsterixDB is a new, full-function BDMS (Big Data Management System) with a feature set that distinguishes it from other platforms in today's open source Big Data ecosystem. Its features make it well-suited to applications like web data warehousing, social data storage and analysis, and other use cases related to Big Data. AsterixDB has a flexible NoSQL style data model; a query language that supports a wide range of queries; a scalable runtime; partitioned, LSM-based data storage and indexing (including B+-tree, R-tree, and text indexes); support for external as well as natively stored data; a rich set of built-in types; support for fuzzy, spatial, and temporal types and queries; a built-in notion of data feeds for ingestion of data; and transaction support akin to that of a NoSQL store. Development of AsterixDB began in 2009 and led to a mid-2013 initial open source release. This paper is the first complete description of the resulting open source AsterixDB system. Covered herein are the system's data model, its query language, and its software architecture. Also included are a summary of the current status of the project and a first glimpse into how AsterixDB performs when compared to alternative technologies, including a parallel relational DBMS, a popular NoSQL store, and a popular Hadoop-based SQL data analytics platform, for things that both technologies can do. Also included is a brief description of some initial trials that the system has undergone and the lessons learned (and plans laid) based on those early "customer" engagements.

==> data.tex <==
%\section{Data}
%
%\subsection{MugshotUsers}

\begin{figure}[htb]
\lstinputlisting[breaklines,breakatwhitespace]{data/shorter-msu.adm.txt}
\vspace{-1mm}
\caption{Mugshot Users}
\end{figure}

%\subsection{MugshotMessages}
\vspace{-4mm}
\begin{figure}[htb]
\lstinputlisting[breaklines,breakatwhitespace]{data/shorter-msm.adm.txt}
\vspace{-1mm}
\caption{Mugshot Messages}
\end{figure}


==> lessons.tex <==
\subsubsection{Lessons learned}

\eat{
\begin{itemize}
\item job creation overhead---Hadoop problem on microscopic level
\item single partition queries / lazy activation (just-in-time query processing)
\end{itemize}

In this section we try to outline some of the important challenges we are attempting to tackle in AsterixDB. 
They have mainly shown up during the performance study, we conducted on AsterixDB.

As briefly shown in Section \ref{sec:perf}, job creation could have a significant overhead in AsterixDB. 
This overhead is considerable for short jobs, and it happens because AsterixDB needs to fully compile each query, it receives, separately; a process that goes through all compilation, and optimization steps, and eventually creates a Hyracks job specification. 
But there are known techniques in data management systems that could be exploited to process repeated, similar queries with high efficiency. 
Relational databases have been using prepared statements and parameterized queries for this purpose, for a long time. Similar features can be built in AsterixDB as well to reduce cost of job generation for frequent known requests.

As of now, AsterixDB routes every query to all partitions of a Dataset.
But there are situations where based on the characteristics of a query and the data placement scheme in the system, the query could avoid running on all partitions. This can improve total throughput of the system, for less resources would be used by a running query. Queries that use primary key of a Dataset are an example of this class. 
AsterixDB uses the primary key to hash partition a Dataset across cluster nodes. Thus for a primary key lookup, compiler can infer about the partition that (potentially) stores relevant data for this query, based on the key. There are more well-studied, advanced query routing techniques that can be used for more complex queries for this matter. 
}

There were 2 main lessons learned/issues discovered while running the performance study.
The first one, the impact of the job creation overhead, was briefly shown in Section \ref{sec:perf}. 
It is essentially the ``Hadoop problem'' at a microscopic level.
For each request a new job is created and executed.
As job creation includes the translation and optimization of an AQL program and execution includes the distribution and start of the job on all cluster nodes, this overhead can be significant for small jobs.
To alleviate this problem we are currently considering an approach that re-uses an existing job---similar to prepared statements in relational databases.

Another problem is that AsterixDB currently routes every request to all partitions of a Dataset.
This is necessary for some requests, but there also are requests for which the system can statically determine that only a subset of the partitions is needed to produce the result.
A trivial example for such requests is the lookup of a record by primary key.
For these requests the evaluation uses significantly more resources than required and thus reduces the system's throughput unnecessarily.
Here we are investigating an approach that lazily activates job on partitions as data from these partitions is needed.


==> operators.tex <==
\section{Operators and Connectors}
%Here we show a complete list of operators: \\
\noindent $\bullet$ AbstractOperatorDescriptor \\
\hspace*{7pt} $\bullet$ HashGroupOperatorDescriptor \\
\hspace*{7pt} $\bullet$ GraceHashJoinOperatorDescriptor \\
\hspace*{7pt} $\bullet$ HybridHashJoinOperatorDescriptor \\
\hspace*{7pt} $\bullet$ InMemoryHashJoinOperatorDescriptor \\
\hspace*{7pt} $\bullet$ NestedLoopJoinOperatorDescriptor \\
\hspace*{7pt} $\bullet$ OptimizedHybridHashJoinOperatorDescriptor \\
\hspace*{7pt} $\bullet$ MaterializingOperatorDescriptor \\
\hspace*{7pt} $\bullet$ SplitVectorOperatorDescriptor \\
\hspace*{7pt} $\bullet$ ExternalSortOperatorDescriptor \\
\hspace*{7pt} $\bullet$ InMemorySortOperatorDescriptor \\
\hspace*{7pt} $\bullet$ OptimizedExternalSortOperatorDescriptor \\
\hspace*{7pt} $\bullet$ UnionAllOperatorDescriptor \\
\hspace*{7pt} $\bullet$ AbstractSingleActivityOperatorDescriptor \\
\hspace*{14pt} $\bullet$ MapperOperatorDescriptor \\
\hspace*{14pt} $\bullet$ ReducerOperatorDescriptor \\
\hspace*{14pt} $\bullet$ FileRemoveOperatorDescriptor \\
\hspace*{14pt} $\bullet$ FileScanOperatorDescriptor \\
\hspace*{14pt} $\bullet$ FrameFileWriterOperatorDescriptor \\
\hspace*{14pt} $\bullet$ PlainFileWriterOperatorDescriptor \\
\hspace*{14pt} $\bullet$ PreclusteredGroupOperatorDescriptor \\
\hspace*{14pt} $\bullet$ DeserializedMapperOperatorDescriptor \\
\hspace*{14pt} $\bullet$ ConstantTupleSourceOperatorDescriptor \\
\hspace*{14pt} $\bullet$ IdentityOperatorDescriptor \\
\hspace*{14pt} $\bullet$ LimitOperatorDescriptor \\
\hspace*{14pt} $\bullet$ NullSinkOperatorDescriptor \\
\hspace*{14pt} $\bullet$ PrinterOperatorDescriptor \\
\hspace*{14pt} $\bullet$ SplitOperatorDescriptor \\
\hspace*{14pt} $\bullet$ ResultWriterOperatorDescriptor \\
\hspace*{14pt} $\bullet$ DataGenOperatorDescriptor \\
\hspace*{14pt} $\bullet$ HDFSReadOperatorDescriptor \\
\hspace*{14pt} $\bullet$ HDFSWriteOperatorDescriptor \\
\hspace*{14pt} $\bullet$ HDFSReadOperatorDescriptor \\
\hspace*{14pt} $\bullet$ HDFSWriteOperatorDescriptor \\
\hspace*{14pt} $\bullet$ BinaryTokenizerOperatorDescriptor \\
\hspace*{14pt} $\bullet$ AbstractDeserializedFileScanOperatorDescriptor \\
\hspace*{21pt} $\bullet$ RecordFileScanOperatorDescriptor \\
\hspace*{14pt} $\bullet$ AbstractFileWriteOperatorDescriptor \\
\hspace*{21pt} $\bullet$ HadoopWriteOperatorDescriptor \\
\hspace*{21pt} $\bullet$ LineFileWriteOperatorDescriptor \\
\hspace*{14pt} $\bullet$ AbstractHadoopOperatorDescriptor \\
\hspace*{21pt} $\bullet$ HadoopMapperOperatorDescriptor \\
\hspace*{21pt} $\bullet$ HadoopReducerOperatorDescriptor \\
\hspace*{14pt} $\bullet$ AbstractIndexOperatorDescriptor \\
\hspace*{21pt} $\bullet$ AbstractLSMInvertedIndexOperatorDescriptor \\
\hspace*{28pt} $\bullet$ LSMInvertedIndexBulkLoadOperatorDescriptor \\
\hspace*{28pt} $\bullet$ LSMInvertedIndexCompactOperator \\
\hspace*{28pt} $\bullet$ LSMInvertedIndexCreateOperatorDescriptor \\
\hspace*{28pt} $\bullet$ LSMInvertedIndexInsertUpdateDeleteOperator \\
\hspace*{28pt} $\bullet$ LSMInvertedIndexSearchOperatorDescriptor \\
\hspace*{21pt} $\bullet$ AbstractTreeIndexOperatorDescriptor \\
\hspace*{28pt} $\bullet$ IndexDropOperatorDescriptor \\
\hspace*{28pt} $\bullet$ TreeIndexBulkLoadOperatorDescriptor \\
\hspace*{28pt} $\bullet$ TreeIndexDiskOrderScanOperatorDescriptor \\
\hspace*{28pt} $\bullet$ TreeIndexInsertUpdateDeleteOperatorDescriptor \\
\hspace*{28pt} $\bullet$ TreeIndexStatsOperatorDescriptor \\
\hspace*{28pt} $\bullet$ LSMTreeIndexCompactOperatorDescriptor \\ 
\hspace*{28pt} $\bullet$ LSMTreeIndexInsertUpdateDeleteOperatorDescriptor \\
\hspace*{28pt} $\bullet$ RTreeSearchOperatorDescriptor \\
\hspace*{28pt} $\bullet$ BTreeSearchOperatorDescriptor \\
\hspace*{35pt} $\bullet$ BTreeUpdateSearchOperatorDescriptor \\

%Below, you can see a complete list of connectors: \\
\noindent  $\bullet$ AbstractConnectorDescriptor \\
\hspace*{7pt} $\bullet$ OneToOneConnectorDescriptor \\
\hspace*{7pt} $\bullet$ AbstractMToNConnectorDescriptor \\
\hspace*{14pt} $\bullet$ HashPartitioningShuffleConnectorDescriptor \\
\hspace*{14pt} $\bullet$ LocalityAwareMToNPartitioningConnectorDescriptor \\
\hspace*{14pt} $\bullet$ MToNPartitioningConnectorDescriptor \\
\hspace*{14pt} $\bullet$ MToNPartitioningMergingConnectorDescriptor \\
\hspace*{14pt} $\bullet$ MToNReplicatingConnectorDescriptor \\
